Analysis of collision avoidance manoeuvres using aerodynamic drag for the Flying Laptop satellite

Collision avoidance is a topic of growing importance for any satellite orbiting Earth. Especially those satellites without thrusting capabilities face the problem of not being able to perform impulsive collision avoidance manoeuvres. For satellites in Low Earth Orbits, though, perturbing accelerations due to aerodynamic drag may be used to influence their trajectories, thus offering a possibility to avoid collisions without consuming propellant. Here, this manoeuvring option is investigated for the satellite Flying Laptop of the University of Stuttgart, which orbits the Earth at approximately 600 km. In a first step, the satellite is aerodynamically analysed making use of the tool ADBSat. By employing an analytic equation from literature, in-track separation distances can then be derived following a variation of the ballistic coefficient through a change in attitude. A further examination of the achievable separation distances proves the feasibility of aerodynamic collision avoidance manoeuvres for the Flying Laptop for moderate and high solar and geomagnetic activity. The predicted separation distances are further compared to flight data, where the principle effect of the manoeuvre on the satellite trajectory becomes visible. The results suggest an applicability of collision avoidance manoeuvres for all satellites in comparable and especially in lower orbits than the Flying Laptop, which are able to vary their ballistic coefficient.

==> setup_commands.tex <==
% ############
% # COMMANDS #
% ############
% Eigene Befehle eignen sich gut um Abkürzungen für lange Befehle zu erstellen. Die Syntax ist folgende:

% \newcommand{neuer Befahl}{ein langer Befehl}
\DeclareMathOperator\erf{erf}
\renewcommand{\phi}{\varphi}
\renewcommand{\epsilon}{\varepsilon}


\newcommand{\euler}{\mathrm{e}} 	% Euler number
\newcommand{\imag}{\mathrm{i}} 		% imaginary unit

\newcommand{\D}{\, \mathrm{d}}


\def\etal{et~al.\xspace} % and others, and co-workers
\def\eg{e.g.,\xspace} % for example
\def\ie{i.e.,\xspace} % that is, in other words
\def\etc{etc} % and other things, and so forth
\def\cf{cf.\xspace} % compare
\def\viz{viz.\xspace} % namely, precisely
\def\vs{vs.\xspace} % against
\def\tca{t_{ca}\xspace}

\newcommand{\flp}{\emph{Flying Laptop}\xspace}

% Vectors and matrices
\renewcommand{\v}[1]{\boldsymbol{#1}}
\newcommand{\m}[1]{\boldsymbol{#1}}
\newcommand{\vect}[1]{\ensuremath{\begin{pmatrix} #1 \end{pmatrix}}}
\newcommand{\mat}[1]{\ensuremath{\begin{bmatrix} #1 \end{bmatrix}}}
\newcommand{\transp}[1]{\ensuremath{#1^{\text{T}}}}

\newcommand{\code}[1]{\texttt{#1}}

\newcommand{\todoil}[1]{\todo[inline]{#1}}
%\newcommand{\cfootnote}{\textcolor{black}{\arabic{footnote}}}

==> setup_packages.tex <==
%%% For including figures, graphicx.sty has been loaded in
%%% elsarticle.cls. If you prefer to use the old commands
%%% please give \usepackage{epsfig}
%
%%% The amssymb package provides various useful mathematical symbols
\usepackage{amssymb}
%%% The amsthm package provides extended theorem environments
\usepackage{amsthm}
\usepackage{amsmath}
\usepackage{mathtools}
%
%\usepackage{chemformula}
%
\usepackage{siunitx}
\sisetup{exponent-product=\ensuremath{\cdot}}
\graphicspath{{images}} 
\usepackage[font=small,labelfont=bf,labelsep=endash,format=plain]{caption}
\usepackage{subcaption}
\renewcommand{\arraystretch}{1.2}
%
\usepackage{tikz}					% Erstellen von Vektorgrafiken in LaTeX
%\usetikzlibrary{matrix, shapes.geometric, arrows, positioning, external, decorations.fractals,%
%	decorations.shapes,%
%	decorations.text,%
%	decorations.pathmorphing,%
%	decorations.pathreplacing,%
%	decorations.footprints,%
%	decorations.markings}
%%\tikzstyle{io} = [trapezium, trapezium left angle=70, trapezium right angle=110, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=blue!30]
%%\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, text width=6.5cm, draw=black, rounded corners=0.2cm]
%%\tikzstyle{process2} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, text width=3cm, draw=black, rounded corners=0.2cm]
%%\tikzstyle{decision} = [diamond, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=green!30]
%%\tikzstyle{arrow} = [thick,->,>=stealth]
%\usepackage{varwidth}
%\newcommand{\umbruch}[2][3cm]{\begin{varwidth}{#1}\centering#2\end{varwidth}}
%
%
%
\usepackage{doi}					% Eingabe von DOI-Nummer mit \doi{ }
\renewcommand{\doitext}{ }
\usepackage{xspace}
%
\usepackage[]{url} 					% Eingabe von URLs mit \url{ }
\urlstyle{same}
%\PassOptionsToPackage{hyphens}{url}
\usepackage[]{hyperref}
\hypersetup{
	%hidelinks,
	colorlinks,
	%citecolor=black,
	%filecolor=black,
	%linkcolor=black,
	%urlcolor=black
}
\usepackage[nameinlink,capitalize]{cleveref}
%
% Für Gleitposition H
\usepackage{float}
\renewcommand\floatpagefraction{.1}
% Multirow in Tabellen:
% Ermöglicht das Verbinden von Zeilen in Tabellen
\usepackage{multirow}
% Für schöne Tabellen, bietet dicke/dünne Linien an
% mehr Tabelleneinstellungen ( \toprule / \midrule / \bottomrule)
\usepackage{booktabs}
\usepackage{tabularx,ragged2e}
\newcolumntype{C}{>{\Centering}X}    % centered version of X column type
%\newcolumntype{L}{>{\RaggedRight}X}  % ragged-right version of X col. type
\renewcommand{\arraystretch}{1.3}		% Erhöht den Zeilenabstand von Tabellen leicht (Ästhetik)
\setlength{\tabcolsep}{5pt}
% Beide Pakete werden für die Ausrichtung der Tabellenspalten benötigt
\usepackage{array}
% Für lange Tabellen
\usepackage{longtable}
\usepackage{rotating}

% for Biblatex
\usepackage{csquotes}
\usepackage{xpatch}
% Schriftart: Latin Modern
\usepackage{lmodern}
% Mehr Farben als den Standard
%\usepackage{usenames,dvipsnames,table,xcdraw]{xcolor}
\usepackage[obeyFinal]{todonotes}
\setlength{\marginparwidth}{1cm}

%% The lineno packages adds line numbers. Start line numbering with
%% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
%% for the whole article with \linenumbers.
%% \usepackage{lineno}

%\usepackage{pgf}
\usepackage{adjustbox}
